European Quantum Ecosystems -- Preparing the Industry for the Quantum Security and Communications Revolution

There is mounting evidence that a second quantum revolution based on the technological capabilities to detect and manipulate single quantum particles (e.g., electrons, photons, ions, etc), a feat not achieved during the first quantum revolution, is progressing fast. It is expected that in less than 10 years, this second quantum revolution shall have a significant impact over numerous industries, including finance, medicine, energy, transportation, etc. Quantum computers threaten the status quo of cybersecurity, due to known quantum algorithms that can break asymmetric encryption, which is what gives us the ability to communicate securely using a public channel. Considering the world's dependence on digital communication through data exchange and processing, retaining the ability to communicate securely even once quantum computers come into play, cannot be stressed enough. Two solutions are available: Quantum Key Distribution (QKD) and Post-Quantum Cryptography (PQC); which, we emphasise, are not mutually exclusive. The EuroQCI initiative, of which EQUO is a part of, focuses on QKD and aims to build a network whereby EU countries can communicate securely through QKD. To this aim, the DEP (Digital Europe Programme) project aims to bring technological matureness to QKD by deploying a QKD test network and, through this exercise, understand what is lacking from an operator's point of view when the time to integrate QKD in their network comes.

==> Makefile <==
.PHONY: default all build embed_fonts clean

PROJECT_NAME = qcnc2024
ROOT_FILE = main.tex
OUT_FILE = $(PROJECT_NAME).pdf

# Final targets
default: build

all: embed_fonts

diff:
	latexpand --explain --expand-bbl build/main.bbl \
		--output build/temp_single_source.tex main.tex
	latexdiff \
		submission/source.tex \
		build/temp_single_source.tex > build/diff.tex
	latexmk -output-directory=build/ -pdf build/diff.tex
	gs -q -dNOPAUSE -dBATCH -dPrinted=false -dPDFSETTINGS=/prepress \
		-sDEVICE=pdfwrite -sOutputFile=diff.pdf build/diff.pdf

# Compilation
build: $(ROOT_FILE)
	@latexmk -halt-on-error -output-directory=build -synctex=1 -pdf $<
	@cp build/$(basename $^).pdf $(OUT_FILE)

# Font embedding rule
embed_fonts: build
	@rm $(OUT_FILE)
	@gs -q -dNOPAUSE -dBATCH -dPrinted=false -dPDFSETTINGS=/prepress \
		-sDEVICE=pdfwrite -sOutputFile=$(OUT_FILE) build/main.pdf

# Cleanup
clean:
	@rm -rf build/
	@rm -f $(OUT_FILE)
	@echo "Clean complete"

